TBCOV: Two Billion Multilingual COVID-19 Tweets with Sentiment, Entity, Geo, and Gender Labels

The widespread usage of social networks during mass convergence events, such as health emergencies and disease outbreaks, provides instant access to citizen-generated data that carry rich information about public opinions, sentiments, urgent needs, and situational reports. Such information can help authorities understand the emergent situation and react accordingly. Moreover, social media plays a vital role in tackling misinformation and disinformation. This work presents TBCOV, a large-scale Twitter dataset comprising more than two billion multilingual tweets related to the COVID-19 pandemic collected worldwide over a continuous period of more than one year. More importantly, several state-of-the-art deep learning models are used to enrich the data with important attributes, including sentiment labels, named-entities (e.g., mentions of persons, organizations, locations), user types, and gender information. Last but not least, a geotagging method is proposed to assign country, state, county, and city information to tweets, enabling a myriad of data analysis tasks to understand real-world issues. Our sentiment and trend analyses reveal interesting insights and confirm TBCOV's broad coverage of important topics.

==> figs_tables.tex <==
\section*{Figures \& Tables}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\textwidth]{figs/weekly_all_tweets_dist.pdf}
% \caption{Weekly distribution of 2,014,792,896 tweets from February \nth{1}, 2020 to March \nth{31}, 2021.}
% \label{fig:data_daily_dist}
% \end{figure}

% \begin{table}[!h]
% \centering
% \begin{tabularx}{\linewidth}{L} 
% \footnotesize
% %\textbf{Col1} 
% \toprule
% Argentina Coronavirus, Armenia Coronavirus, Australia Coronavirus, Austria Coronavirus, Azerbaijan Coronavirus, Bahamas Coronavirus, Bahrain Coronavirus, Bangladesh Coronavirus, Barbados Coronavirus, Belarus Coronavirus, Belgium Coronavirus, Belize Coronavirus, Benin Coronavirus, Bhutan Coronavirus, Bolivia Coronavirus, Bosnia Herzegovina Coronavirus, Botswana Coronavirus, Brazil Coronavirus, Brunei Coronavirus, Bulgaria Coronavirus, Burkina Coronavirus, Burundi Coronavirus, Cambodia Coronavirus, Cameroon Coronavirus, Canada Coronavirus, COVID-19, Congo COVID-19, Congo COVID-19, Costa Rica COVID-19, Croatia COVID-19, Cuba COVID-19, Cyprus COVID-19, Czech Republic COVID-19, Denmark COVID-19, Djibouti COVID-19, Dominica COVID-19, Dominican Republic COVID-19, East Timor COVID-19, Ecuador COVID-19, Egypt COVID-19, El Salvador COVID-19, Equatorial Guinea COVID-19, Eritrea COVID-19, Estonia COVID-19, Ethiopia COVID-19, Fiji COVID-19, Finland COVID-19, France COVID-19, Gabon COVID-19, Gambia COVID-19, Georgia COVID-19, Germany COVID-19, Ghana COVID-19, \#socialdistancing us, \#socialdistancing usa, \#socialdistancing Alabama, \#socialdistancing Alaska, \#socialdistancing Arizona, \#socialdistancing Arkansas, \#socialdistancing California, \#socialdistancing Colorado, \#socialdistancing Connecticut, \#socialdistancing Delaware, \#socialdistancing Florida, \#socialdistancing Georgia, \#socialdistancing Hawaii, \#socialdistancing Idaho, \#socialdistancing Illinois, \#socialdistancing Indiana, \#socialdistancing Iowa, \#socialdistancing Kansas, \#socialdistancing Kentucky, \#socialdistancing Louisiana, \#socialdistancing Maine, \#socialdistancing Maryland, \#socialdistancing Massachusetts, \#socialdistancing Michigan, económica, quédate en casa Colombia, respiradores Colombia, tapabocas Colombia, UCI disponibles, recuperados covid19 Colombia, muertes Colombia, Nariño Coronavirus, Nariño Covid19, \#coronavirus, \#Corona, \#COVID19, \#WuhanCoronavirus, \#ncoV2019, \#coronavirus, Italia, lombardia, \#covid19italia, \#COVID19Pandemic, covid, \#CoronavirusAustralia, \#pandemic, covid-19 usa\\
% \bottomrule
% \end{tabularx}
% \caption{A sample of keywords/hashtags used for data collection}
% \label{tab:collection_terms}
% \end{table}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\textwidth]{figs/lang_dist_2.pdf}
% \caption{Distribution of languages with more than 10K tweets. Number of tweets on y-axis (log-scale).}
% \label{fig:lang_dist}
% \end{figure}


% \begin{table}[!h]
% \centering
% \begin{minipage}[b]{0.40\columnwidth}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lr}
%  \toprule
% Users (unique)  & \# of tweets \\ 
%  \midrule
% Unique users in the dataset & 87,771,834  \\
% Users with at least one geo tweet & 346,394   \\
% Users with at least one place tweet & 3,532,827  \\
% Users with valid user location value & 22,851,095  \\
%  \bottomrule
% \end{tabular}
% }
% \caption{User-related statistics}
% \label{tbl:users_unique_stats}
% \end{minipage}
% %\hfill % 
% \begin{minipage}[b]{0.40\columnwidth}
% \centering
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{lr} 
%  \toprule
% Verified users (unique)  & \# of tweets \\ 
%  \midrule
% Verified users in the dataset & 268,642  \\
% Verified users with at least one geo tweet & 4,342  \\
% Verified users with at least one place tweet & 39,025   \\
% Verified users with valid user location value & 165,706 \\
%  \bottomrule
% \end{tabular}
% }
% \caption{Statistics related to verified users}
% \label{tbl:verified_users_stats}
% \end{minipage}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{lrrrr}
% \toprule
% \multicolumn{1}{l}{\textbf{Language}} & \multicolumn{1}{r}{\textbf{Person}} & \multicolumn{1}{r}{\textbf{Organization}} & \multicolumn{1}{r}{\textbf{Location}} & \multicolumn{1}{r}{\textbf{Miscellaneous}}\\
% \midrule
% English (U) & 14,796,271 & 18,887,285 & 2,930,148 & 10,798,850 \\
% English (A) & 409,794,668 & 611,669,779 & 483,680,780 & 1,690,122,455\\
% Spanish (U) & 3,777,463 & 2,230,017 & 3,265,204 & 14,968,547\\
% Spanish (A) & 98,561,105 & 69,581,078 & 169,903,131 & 301,512,355\\
% Portuguese (U) & 1,439,192 & 932,504 & 1,006,396 & 2,845,321 \\
% Portuguese (A) & 27,577,759 & 15,896,880 & 40,090,891 & 52,440,351\\
% French (U) & 1,374,884 & 804,336 & 719,896 & 3,894,968\\
% French (A) & 23,595,420 & 17,256,551 & 34,064,424 & 63,010,283\\
% \midrule
% Total (U) & \textbf{55,721,884} & \textbf{33,324,173} & \textbf{10,336,415} & \textbf{40,767,983}\\
% Total (A) & \textbf{803,832,752} & \textbf{814,205,050} & \textbf{805,175,906} & \textbf{2,320,195,791}\\
% \bottomrule
% \end{tabular}
% \caption{Named-entities extraction results for the top four languages. `U' denotes ``unique occurrences'' and `A' denotes ``all occurrences'' of entities.}
% \label{tab:entities_4langs}
% \end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{lrrrrrrr}
% \toprule
% \multicolumn{1}{l}{Location attribute} & \multicolumn{1}{r}{Total occurrences} & \multicolumn{1}{r}{Geotagged (yield \%)} & \multicolumn{1}{r}{Countries} & \multicolumn{1}{r}{States} & \multicolumn{1}{r}{Counties} & \multicolumn{1}{r}{Cities}\\
% \midrule
% Geo coordinates & 2,799,378 & 2,799,378 (100\%) & 211 & 1,912 & 9,037 & 8,079\\
% Place & 51,411,442 & 51,061,938 (99\%) & 215 & 1,906 &13,343 & 9,932\\
% User location & 1,284,668,011 & 1,132,595,646 (88\%) & 218 & 2,511 & 24,806 & 20,648\\
% User profile description & 1,642,116,879 & 180,508,901 (11\%)& 218 & 2,485 & 18,588 & 14,600\\
% Tweet text & 2,014,792,896 & 515,802,081 (26\%)& 218 & 2,513 & 24,235 & 20,549\\
% \bottomrule
% \end{tabular}
% \caption{Geotagging results for all five attributes with unique occurrences, geotagging yield, and resolved countries, states, counties, and cities}
% \label{tab:geotagging_results}
% \end{table}


% \begin{figure}[!h]
% \centering   
% \subfigure[Monthly proportion of tweets from top-10 countries]{\label{fig:top10_countries_dist}\includegraphics[width=0.815\columnwidth]{figs/top_10_countries.pdf}}
% \subfigure[Monthly proportion of tweets from top-10 cities]{\label{fig:top10_cities_dist}\includegraphics[width=0.815\columnwidth]{figs/top_10_cities.pdf}}%\vspace{-0.4cm}
% \caption{Countries and cities distributions across months sorted by their overall tweets}
% \label{fig:top_10_countries_citites}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.95\textwidth]{figs/worldwide_normalized_tweets.pdf}%\vspace{-0.4cm}
% \caption{Geotagged tweets worldwide normalized by country's population (per 100,000 persons). Tweets geotagged using \textit{user location}, \textit{user profile description}, and \textit{GPS-coordinates} are used.}
% \label{fig:worldwide_tweets_normalized}
% \end{figure}


% \begin{table}[!h]
% \centering
% \caption{Named-entity recognition results from tweet text and usernames}
% \label{tab:entities_stats}
% \begin{tabular}{lrr}
% \toprule
% Entity type & Extractions from tweet text & Extractions from usernames \\
% \midrule
% Person & 2,763,063,834 & 1,242,674,026 \\
% Organization & 1,106,904,014 & 758,547,010 \\
% Location & 858,159,860 & 297,212,754 \\
% Misc & 15,281,791 & 10,116,324\\
% \bottomrule
% \end{tabular}
% \end{table}

% %%%%%%%%%%%%%%% Geo inferrence
% \begin{table}[!h]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% {\bf Tweet field} & {\bf Country} & {\bf State} & {\bf County} & {\bf City}\\
% \midrule
% User location  & 0.901 (7527) & 0.831 (7099) & 0.656 (5001) & 0.689 (3492)\\ 
% Tweet text & 0.780 (3028)   & 0.719 (2799)  & 0.615 (1752) & 0.611 (1490)\\ 
% User profile description & 0.700 (1906) & 0.384 (1686) & 0.384 (1153) & 0.563 (751)\\
% Place &  0.988 (7990) & 0.967 (7871) & 0.771 (7394)  & 0.967 (4903)\\
% \bottomrule
% \end{tabular}
% \caption{Accuracy of the geotagging approach at different granularity levels. Numbers in the parenthesis represent tweets sample.}
% \label{tbl:eval}
% \end{table}




%%%%%%%%%%%%%%% Sentiment
% \begin{figure}[!h]
% \centering
% \includegraphics[width=\textwidth]{figs/worldwide_sent.pdf}
% \caption{Weekly distribution representing public sentiment based on worldwide tweets in all languages.}
% \label{fig:world_weekly_sent}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\textwidth]{figs/world_sentiment_map.pdf}
% \caption{Worldwide sentiment based on normalized classifier scores of the representative sentiment in each country. Numbers on countries are z-scores computed using the representative sentiment tweets normalized by total tweets from all countries.}
% \label{fig:world_sentiment_map}
% %\Description{Tweets sentiment scores for each country obtained using a multilingual transformer model trained on million of tweets.}
% \end{figure}

% \begin{figure}[!h]
% \centering    
% \subfigure[United States]{\label{fig:us_sent}\includegraphics[width=0.49\columnwidth]{figs/us_sent.pdf}}
% \subfigure[United Kingdom]{\label{fig:uk_sent}\includegraphics[width=0.49\columnwidth]{figs/uk_sent.pdf}}
% \subfigure[India]{\label{fig:india_sent}\includegraphics[width=0.49\columnwidth]{figs/india_sent.pdf}}
% %\subfigure[Italy]{\label{fig:italy_sent}\includegraphics[width=0.49\columnwidth]{figs/italy_sent.pdf}}
% \subfigure[Canada]{\label{fig:canada_sent}\includegraphics[width=0.49\columnwidth]{figs/canada_sent.pdf}}
% \subfigure[Brazil]{\label{fig:brazil_sent}\includegraphics[width=0.49\columnwidth]{figs/brazil_sent.pdf}}
% \subfigure[Spain]{\label{fig:spain_sent}\includegraphics[width=0.49\columnwidth]{figs/spain_sent.pdf}}\vspace{-0.4cm}
% \caption{Weekly distribution of sentiment labels for the top six countries}
% \label{fig:countries_weekly_sent}
% \end{figure}


% \begin{figure}[!h]
% \centering    
% \subfigure[United States positive sentiment]{\label{fig:us_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/us_pos_sent_box.pdf}}
% \subfigure[United States negative sentiment]{\label{fig:us_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/us_neg_sent_box.pdf}}
% \subfigure[United Kingdom positive sentiment]{\label{fig:uk_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/uk_pos_sent_box.pdf}}
% \subfigure[United Kingdom negative sentiment]{\label{fig:uk_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/uk_neg_sent_box.pdf}}
% \subfigure[India positive sentiment]{\label{fig:india_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/india_pos_sent_box.pdf}}
% \subfigure[India negative sentiment]{\label{fig:india_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/india_neg_sent_box.pdf}}
% % \subfigure[Italy positive sentiment]{\label{fig:italy_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/italy_pos_sent_box.pdf}}
% % \subfigure[Italy negative sentiment]{\label{fig:italy_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/italy_neg_sent_box.pdf}}
% \subfigure[Canada positive sentiment]{\label{fig:canada_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/canada_pos_sent_box.pdf}}
% \subfigure[Canada negative sentiment]{\label{fig:canada_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/canada_neg_sent_box.pdf}}
% \subfigure[Brazil positive sentiment]{\label{fig:brazil_pos_sent_box}\includegraphics[width=0.45\columnwidth]{figs/brazil_pos_sent_box.pdf}}
% \subfigure[Brazil negative sentiment]{\label{fig:brazil_neg_sent_box}\includegraphics[width=0.45\columnwidth]{figs/brazil_neg_sent_box.pdf}}
% \caption{Monthly distribution summary of positive and negative sentiment tweets for the top five countries}
% \label{fig:countries_sent_box}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=0.95\textwidth]{figs/us_counties_sentiment.pdf}\vspace{-0.4cm}
% \caption{Sentiment across US counties. Tweets geotagged using \textit{user location}, \textit{user profile description}, and \textit{GPS-coordinates} are used after normalizing by the total number tweets from each county.}
% \label{fig:us_county_sent_map}
% \end{figure}

% \begin{figure}[!h]
% \centering
% \includegraphics[width=\columnwidth]{figs/langs_sentiment.pdf}
% \caption{Weekly distribution of sentiment labels of tweets in four languages (Spanish, Portuguese, French, and Arabic).}
% \label{fig:langs_sentiment}
% \end{figure}

%%%%%%%%%%%% Gender map (female %)
% \begin{figure}[!h]
% \centering
% \includegraphics[width=\columnwidth]{figs/female_users_compressed.pdf}
% \caption{Percentage of female users for countries meeting representative sampling criteria (confidence interval=95\%; margin of error$\leq1\%$). Gray color indicates the countries excluded due to under representation ($N=85$).}
% \label{fig:female_users}
% \end{figure}


%%%%%%%%%%%% Digital divide map
% \begin{figure}[!h]
% \centering
% \includegraphics[width=\textwidth]{figs/digital_divide.pdf}
% \caption{Global digital divide estimated through the type of device used for tweeting. Representative device type penetration (percentage) is shown on top of each country.}
% \label{fig:digital_divide_map}
% \end{figure}


%%%%%%%%%%%%%%%%%%% Trends
% \begin{table}[!h]
% \centering

% \footnotesize
% \begin{tabular}{ll}
% \toprule
% \textbf{Topics representing different issues} & \textbf{Sub-topics related to the main topic} \\
% \midrule
% COVID-19 symptoms & Fever, cough, shortness of breath, headache, loss of taste and smell \\
% COVID deaths mentions & Parents, siblings, grandparents, relatives, and close connections \\
% Food shortages & Food availability, food access, food adequacy, and food acceptability \\
% Anxiety \& depression & Anger, sleepless, fearful, upset, restless, and anxious\\
% Mask usage \& importance & Mask violation, masks are important, wear masks, masks save lives, masks useless\\
% Willingness to take/taken vaccine & Reactions to vaccine, harmful vaccine, got vaccine, covid jab taken, will take vaccine\\
% \bottomrule
% \end{tabular}
% \caption{Term groups of four topics for trend analysis}
% \label{tab:trend_groups}
% \end{table}


% \begin{figure}[!h]
% \centering    
% \subfigure[COVID-19 symptoms]{\label{fig:symptoms_trends}\includegraphics[width=0.49\columnwidth]{figs/symptoms_trend.pdf}}
% \subfigure[Anxiety, anger, sadness]{\label{fig:axiety_trends}\includegraphics[width=0.49\columnwidth]{figs/anxiety_trends.pdf}}
% \subfigure[Parents, siblings, relatives deaths]{\label{fig:deaths_trends}\includegraphics[width=0.49\columnwidth]{figs/covid_deaths_trend.pdf}}
% \subfigure[Food insecurity and shortages]{\label{fig:food_trends}\includegraphics[width=0.49\columnwidth]{figs/food_trends.pdf}}
% \subfigure[Mask usage \& shortages \& importance]{\label{fig:mask_trends}\includegraphics[width=0.49\columnwidth]{figs/mask_trends.pdf}}
% \subfigure[Willingness to take or taken vaccine]{\label{fig:vaccine_trends}\includegraphics[width=0.49\columnwidth]{figs/vaccine_trends.pdf}}\vspace{-0.4cm}
% \caption{Weekly trends of important issues related to personal and social lives of users linked to COVID-19\vspace{-0.1cm}}
% \label{fig:weekly_trends_misc_topics}
% \end{figure}



%%%%%%%%%%%  Geotagging evaluation
% \begin{table}[]
% \centering
% \begin{tabular}{lllll}
% \toprule
%  & \multicolumn{1}{c}{Country} & \multicolumn{1}{c}{State} & \multicolumn{1}{c}{County} & \multicolumn{1}{c}{City} \\
%  \midrule
% Place & 0.988 (7,990) & 0.967 (7,871) & 0.771 (7,394) & 0.967 (4,903)\\
% \bottomrule
% \end{tabular}
% \caption{Geotagging method evaluation of the \textit{place} attribute (in terms of precision). Numbers in parenthesis represent the sampled set.}
% \label{tab:geo_place_evaluation}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{lcccc}
% \toprule
%  \multicolumn{1}{l}{Metric} & \multicolumn{1}{c}{Country} & \multicolumn{1}{c}{State} & \multicolumn{1}{c}{County} & \multicolumn{1}{c}{City} \\
%  \midrule
% Precision & 0.868 & 0.839 & 0.648 & 0.802 \\
% Recall & 1.000 & 0.968 & 0.922 & 0.656 \\
% F1-score & 0.929 & 0.899 & 0.761 & 0.722\\
% \bottomrule
% \end{tabular}
% \caption{Geotagging method evaluation for the \textit{user location} attribute }
% \label{tab:geo_userloc_evaluation}
% \end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{lcccc}
% \toprule
%  \multicolumn{1}{l}{Metric} & \multicolumn{1}{c}{Country} & \multicolumn{1}{c}{State} & \multicolumn{1}{c}{County} & \multicolumn{1}{c}{City} \\
%  \midrule
% Precision & 0.888 & 0.781 & 0.056 & 0.430 \\
% Recall & 0.732 & 0.640 & 0.462 & 0.184 \\
% F1-score & 0.803 & 0.703 & 0.100 & 0.258\\
% \bottomrule
% \end{tabular}
% \caption{Geotagging method evaluation for the text-based attributes (i.e., \textit{tweet text} \& \textit{user profile description})}
% \label{tab:geo_text_evaluation}
% \end{table}




% %%%%%%%%%%%  Gender evaluation

% \begin{table}[!h]
% \centering
  
%   \begin{tabular}{lcccc}
%     \toprule
%     Metric & Female & Male & Macro avg. & Weighted avg.\\
%     \midrule
%     Precision & 0.872 & 0.816 &  0.844 & 0.850 \\
%     Recall & 0.885 & 0.797 & 0.841 & 0.851 \\
%     F1-score & 0.878 & 0.807 & 0.843 & 0.850 \\
%   \bottomrule
% \end{tabular}
% \caption{Gender classification results (model=Random Forest)}
%   \label{tab:gender_eval}
% \end{table}

% \begin{table}[!h]
% \centering
  
%   \begin{tabular}{cccccc}
%     \toprule
%     Metric & Female & Male & Accuracy & Macro avg. & Weighted avg.\\
%     \midrule
%     Precision & 0.872 & 0.816 & 0.851 & 0.844 & 0.850 \\
%     Recall & 0.885 & 0.797 & 0.852 & 0.841 & 0.851 \\
%     F1-score & 0.878 & 0.807 & 0.851 & 0.843 & 0.850 \\
%   \bottomrule
% \end{tabular}
% \caption{Gender classification results (model=Random Forest)}
%   \label{tab:gender_eval}
% \end{table}
